Amortizing Pragmatic Program Synthesis with Rankings

The usage of Rational Speech Acts (RSA) framework has been successful in building \emph{pragmatic} program synthesizers that return programs which, in addition to being logically consistent with user-generated examples, account for the fact that a user chooses their examples informatively. We present a general method of amortizing the slow, exact RSA synthesizer. Our method first query the exact RSA synthesizer to compile a communication dataset. The dataset contains a number of example-dependent rankings of subsets of programs. It then distills a \textit{single} global ranking of all programs as an approximation to every ranking in the dataset. This global ranking is then used at inference time to rank multiple logically consistent candidate programs generated from a fast, non-pragmatic synthesizer. Experiments on two program synthesis domains using our ranking method resulted in orders of magnitudes of speed ups compared to the exact RSA synthesizer, while being more accurate than a non-pragmatic synthesizer when communicating with humans. Finally, we prove that in the special case of synthesis from a single example, this approximation is exact.

==> sections/_global_ranking.tex <==
\section{Global Pragmatic Ranking}
We formally define a global ranking $\sigma_L$ for a listener $L$, and show how it can be used to approximate the pragmatic synthesizer $L_1$ derived from \rsaslow{}.

\paragraph{Global Ranking} 
Given a listener $L(w|u)$, a \emph{global ranking} $\sigma_L$ an ordering of programs such that: % rephrased to not presuppose that a ranking exists
\begin{align}
\label{eqn:global_rank1}
\begin{split}
    \forall w, w', u.~ \textbf{if}~ L(w|u)>0 \wedge L(w'|u)>0. \\ 
    \textbf{then}~L(w|u) > L(w'|u) \iff \sigma_L[w] \succ \sigma_L[w']
\end{split}
\end{align}
Which is to say, for any two competing programs $w, w'$ given example $u$, if both have non-zero probabilities under $L(\cdot|u)$, then \textit{both} $\sigma_L$ and $L(\cdot|u)$ will sort these two programs in the same order.

\paragraph{A global ranking is example agnostic}
The most salient feature of a ranking $\sigma$ is that it is \emph{example agnostic}: the same ranking is used to order all the programs irrespective of the example given. This is counter-intuitive, because one might expect that given different examples $u$, $u'$, it is possible for a listener $L$ to give different rankings for $w$ and $w'$, even if both programs are consistent with both examples:
\begin{align}
\label{eqn:nocycle}
\begin{split}
    L(w|u)>L(w'|u)>0 ~ \wedge ~ L(w'|u')>L(w|u')>0
\end{split}
\end{align}

However, we will show that -- in the case of boolean lexicons with a single example and an RSA listener as described in the previous section -- a global pragmatic ranking $\sigma_L$ consistent with $L$ must exist, and in the case of multiple examples, a global ranking $\tilde{\sigma_L}$ can well approximate the true $L$ ranking empirically.
% Let's validate it: 
% \begin{enumerate}
%   \setlength\itemsep{-0.5em}
%     \item given $u_h$, we only have 1 valid program $w_{HG}$.
%     \item given $u_g$, $L_1(w_{GS}|u_g)>L_1(w_{HG}|u_g)$, and $w_{GS} \succ w_{HG}$.
%     \item given $u_s$, $L_1(w_{S}|u_s)>L_1(w_{GS}|u_s)$, and $w_{S} \succ w_{GS}$.
% \end{enumerate}
% As we can see, a global ranking exists for $L_1$ in our example. In the next section, we will prove this in general.

\paragraph{Rank-based listeners}
Given any ranking $\sigma$, one can use it to construct a \emph{rank based listener} $L_{\sigma} : U \Rightarrow W^*$, that takes in an example $u$ and returns a sorted list of all satisfying programs by progressing through the list of ranked programs in $\sigma$ and filtering for consistency with $u$. As we can see, both the time and space complexity of $L_\sigma$ are $O(|W|)$.

\subsection{This Work: Pragmatic Synthesis using Rankings}
We are now in a position to explain our work -- using a global pragmatic ranking to amortizing the RSA inference. 
Imagine we had a pre-computed, global ranking of programs, we would simply need to find consistent programs and rank them, which requires only $\mathcal{O}(|W|)$ steps. Consider the example from earlier where a speaker provides the example \textsf{\textit{01}}. If we had determined that the global ordering of programs was $\texttt{0\{1\}} \succ \texttt{0+1\{1\}} \succ \texttt{0\{2\}1+} \succ \texttt{0+1*}$, we could identify \texttt{0+1\{1\}} as the most preferred program that was consistent by progressing through the list, and checking consistency. Even after providing a second example \textsf{\textit{001}}, the outcome of this remains unchanged and still correct.
In the rest of this paper, we describe how, for the case of single example (the user can only provide 1 string, e.g. \textsf{\textit{001}}), such a ranking provably exists. And for the case of multiple examples (the user provides multiple strings incrementally, e.g. \textsf{\textit{001}},\textsf{\textit{01}}), even though we may not have guarantees, we empirically verify that we can compute and use such a ranking to make pragmatic program synthesis much more efficient.

==> sections/background_old.tex <==
\section{Background and Motivation}
In this section, we provide background on a reference game framework of program synthesis, which affords building a \emph{pragmatic synthesizer} that can infer a user's intended program from few examples \cite{bool_pu2020program}. We illustrate this framework using a toy example from a small version of the regular expression domain of this work. 
% We then give an informal overview of how one can use a global pragmatic order, the contribution of this paper, to make pragmatic synthesis scalable to more complex domains, such as unrestricted regular expressions.
% building a pragmatic program synthesizer, instantiated on a small regular expression domain. Then, we give an informal overview of how one can use a global pragmatic order, the contribution of this paper, to make it more efficient.
% In this section, we provide an motivating example showing fjkdjlsdkfjklsa how ordering works fjkldsfjl and ordering is awesome and provided nesejsklksary backgrounds for this work. 

% \sv{make this but with regex, hit the following goals, and also keep the notations consistent}
% few goals to hit for this section:

% \begin{enumerate}
%     \item Explain the incremental RSA algorithm on a regex domain
%     \item Show the two steps separately, allowing for the utilization of part of it for a single-utterance example
%     \item create a global ranking of regexes (the process of obtaining it is not necessary to explain, assume it's given), then illustrate how this ranking can be employed to conserve computation time for the resource-intensive computations in previous
% \end{enumerate}



% \subsection{Reference Game}
% % In a reference game, a speaker $S$ attempts to communicate a hypothesis $w$ to the listener $L$ using an utterance $u$. The speaker $S$ is a probability distribution $S(u|w)$, which takes in a hypothesis $w$ and produces an utterance $u$. The listener $L$ is a probability distribution $L(w|u)$, and can recover a hypothesis $w' \sim L(w'|u)$. The communication is successful if $w'=w$.

% We consider a reference game between two players -- a speaker $S$ and a listener $L$ -- where the speaker has to use an utterance $u \in U$ to communicate a hypothesis $w \in W$ to the listener. The speaker chooses the utterance based on a distribution $S(U|W)$, and the listener guesses a hypotheses $w'$ based on $L(W|U=u)$. If $w = w'$, communication is successful.

% \textcolor{red}{SV: describe the goal of maximizing success}

% \paragraph{Measuring Communication Effectiveness}
% The communication game is successful if $w'=w$. This amounts to marginalizing over all possible utterances:
% \[
% P_{success}(w) = \sum_u S(u|w)L(w'=w|u)
% \]
% Given a speaker $S$ and a listener $L$, we define the \emph{average round-trip success rate} as:
% \[
% roundtrip(S,L) = \frac{1}{|W|} \sum_w \sum_u S(u|w)L(w'=w|u)
% \]
% $roundtrip(S,L)$ measures on average, if a hypothesis $w$ is given at random, how likely is the communicative pair $(S,L)$ going to recover it in a reference game.

% \subsection{A Simple Example}

% Consider the following reference game adopted from \cite{goodman2016pragmatic}. There are three hypotheses: A person wearing a hat and glasses $w_{HG}$, a person wearing glasses and a smile $w_{GS}$, and a person smiling $w_S$. There are three utterances: The word ``hat'' $u_h$, the word ``glassess'' $u_g$, and the word ``smile'' $u_s$. The lexicon $M$\footnote{also called a meaning matrix} gives the relationship between the hypotheses and the utterances. In this work, we're interested in boolean lexicons -- those with entries of 1s and 0s denoting whether a pair of utterance and hypothesis $(u,w)$ is consistent (see Figure \ref{fig:example}). In our example, $M[u_h,w_{HG}]=1$ (the utterance ``hat'' is consistent with hypothesis $w_{HG})$ and $M[u_g,w_S]=0$ (the utterance ``glasses'' is inconsistent with the hypothesis $w_S$).

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\columnwidth]{assets/placeholder_example.png} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
% \caption{fdafdasfdsa}
% \label{fig:example}
% \end{figure}

% Consider the problem of finding a regular expression given examples of strings in the regular language it describes. \citet{bool_pu2020program} argue that a program synthesis \cite{some_sumit_gulwani_paper} problem such as this can be viewed as a reference game where the user assumes the role of a speaker and the program synthesizer assumes the role of a listener. The user uses examples of program behavior (strings in the regular language) as utterances to communicate the intended program -- the hypothesis, a regular expression -- to the synthesizer. To build an effective synthesizer, we want to compute a distribution $L(W|U)$ that maximizes the chance of successful communication. 

% Minimally, the listener must produce a program that is \emph{consistent} with the utterances given by the speaker. This consistency is determined by the \emph{lexicon} $M: W \times U \to \mathbb{R}$, which assigns a non-negative \textcolor{red}{SV: Is this a requirement?} real value to each $(w, u)$ pair. We can also view the lexicon as a matrix of real values, or a \emph{meaning matrix}. In the program synthesis case, the lexicon is binary -- every example is either consistent or inconsistent with a particular program. If we have no further information about how the utterances are produced, we might believe that the speaker is equally likely to refer to any of the consistent programs. This strategy resembles a \emph{literal listener} $L_0$ that infers a uniform distribution over all true hypotheses.

% \begin{figure*}
%     \centering
%     \begin{subfigure}{0.19\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{assets/lexicon.png}
%         \caption{}
%         \label{}
%     \end{subfigure}
%     \begin{subfigure}{0.75\textwidth}
%         \begin{subfigure}{\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{assets/rsa_turn_1.png}
%             \caption{}
%             \label{}
%         \end{subfigure}
    
%         \begin{subfigure}{\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{assets/rsa_turn_2.png}
%             \caption{}
%             \label{}
%         \end{subfigure}
%     \end{subfigure}
% \end{figure*}

% \evan{just dumping some phrases here}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.5\columnwidth]{assets/lexicon.png}
%     \caption{A boolean lexicon for a small reference game of regular expressions. The rows are the utterances (strings) and the columns are hypotheses (regexes), and each entry denotes if a string is consistent with a regex.}
%     \label{fig:lexicon}
% \end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[width=\columnwidth]{assets/ranking-pragmatics-listener-matrix.png}
    \caption{A boolean lexicon for a small reference game of regular expressions. The rows are the utterances (strings) and the columns are hypotheses (regexes), and each entry denotes if a string is consistent with a regex.}
    \label{fig:lexicon}
\end{figure}

\subsection{Synthesis as a Reference Game}
Consider the problem where a user gives example strings to a synthesis system, and asks it to find a matching regular expression. This process can be modeled as a \textbf{reference game} \cite{lewis1979scorekeeping},
where a speaker (the user) chooses a few utterances (strings) to give to the listener (the synthesizer), with the intention that the listener can infer the correct hypothesis (regular expression). 
% (Maybe show a figure? regex->user->utter->syntheiszer->recoveredregex). 
This reference game is characterized by the lexicon $M$,
%: U \times W$, which contains pairs $(u, w)$ where the string $u$ belongs to the regular language described by $w$. We can also view this as 
a boolean matrix of 1s and 0s (Figure~\ref{fig:lexicon}). % \daniel{maybe change the ``lexicon'' term; it's a holdover from RSA but might not make sense here?} evan: it's not much overhead of a term, and I use it for the proof so we should keep it
In $M$, each row corresponds to an utterance/example and each column corresponds to a hypothesis/program, and 1s indicating \emph{consistency} of its corresponding utterance and a hypothesis: whether the program (e.g. regular expression) matches the example (e.g. string). As we can see, a given utterance (such as \textsf{\textit{001}}) may be consistent with multiple hypotheses (\texttt{0+\{1\}}, \texttt{0\{2\}1+}, and \texttt{0+1*}).
% \daniel{clarify this is a toy example, and really we have combinatorially large sets of strings and programs}

\subsection{A Literal Program Synthesizer}
% \daniel{super nitpicky, but ``uninformative'' to me conveys a speaker rather than a listener. Maybe just say ``non-pragmatic'', or ``literal''}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.5\columnwidth]{assets/l0_1.png}
%     \caption{Given the utterance \texttt{01}, a naive synthesizer $L_0$ will predict \texttt{0+1\{1\}} and \texttt{0+1*} as equally probable}
%     \label{fig:l0_1}
% \end{figure}

How might we build a system that takes an utterance (say \textsf{\textit{01}}) and produces the intended hypothesis \texttt{0+1\{1\}}?
As \textsf{\textit{01}} is consistent with multiple hypotheses (\texttt{0+1\{1\}} and \texttt{0+1*}), a naive strategy is to treat all consistent hypotheses as equally likely, scaled by a prior distribution of hypotheses $P(w)$:
\begin{align}
    L_0(w|u) & \propto  P(w) M[u,w] \label{eq:l0} \\ 
            & =  P(w) \frac{M[u,w]}{\sum_{w'} M[u,w']}
\end{align}
A synthesizer built this way is a \emph{literal listener} $L_0$ \cite{bergen2016pragmatic}. Assuming the prior $P(w)$ is uniform over programs, we can construct it by normalizing the rows of the matrix $M$, resulting in a probability distribution over hypotheses $W$ given utterances $u$ (Figure). As we can see, given the utterance \textsf{\textit{01}}, this listener predicts an equal probability of \texttt{0+1\{1\}} and \texttt{0+1*} being the intended program.
% However, as \citet{bool_pu2020program} find, end users do not communicate effectively with $L_0$, requiring  longer interactions compared to a model that reasons about how users choose utterances informatively.
% compared to the more pragmatic $L_1$ listener, which we will describe now.
% this does not result in a very effective synthesizer, often failing to successfully interpret the speaker's communication.
% \sv{you might want to make a remark that, the entire $L_0$ matrix, while you can show it fully for this small domain, cannot be explicitly constructed for real program synthesis problems and must be dynamically generated on the fly}

\subsection{A Pragmatic Synthesizer of a Single Example}
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=\columnwidth]{assets/l1_1.png}
%     \caption{The RSA framework performs alternating normalization of the literal listener ($L_0$) distribution in Figure \ref{fig:l0_1} to first derive a pragmatic speaker, $S_1$, which models how a user chooses utterances informatively, and then a pragmatic listener, $L_1$, which models how the synthesizer should infer programs assuming an informative user. Given \texttt{01}, $L_1$ identifies \texttt{0+1\{1\}} as the most probable intended program.
%     % A pragmatic listener, $L_1$, based on the RSA framework is derived by normalizing. Given the string \texttt{01}, it identifies \texttt{0+1\{1\}} as the most probable intended program
%     }
%     \label{fig:l1_1}
% \end{figure}

A key insight to improving on the literal synthesizer is to consider that a user is cooperatively choosing an utterance to be \emph{informative} about the intended program to the synthesizer. The Rational Speech Acts (RSA) framework models this informative choice of utterances using recursive Bayesian reasoning \cite{frank2012predicting}. By reasoning about why a speaker(user) might have chosen a particular utterance(examples), rather than possible alternatives, 
% if they wanted to communicate a particular hypothesis, 
the listener(synthesizer) can disambiguate the hypothesis(program) to which the speaker was referring.
% \daniel{consider standardizing terminology; we're mixing ``hypothesis'', ``regex'', and maybe ``program''}
Formally, the RSA framework produces a chain of alternating listeners and speakers beginning with the $L_0$ model above, each of which reasons about the previous agent.
\begin{align}
    S_1(u|w) &= \frac{L_0(w|u)}{\sum_{u'} L_0(w|u')} \\
    L_1(w|u) &= \frac{S_1(u|w)}{\sum_{w'} S_1(u|w')} \label{eq_rsa}
\end{align}
Applying this framework amounts to normalizing the columns of the $L_0$ matrix to obtain $S_1$, the normalize the rows of $S_1$ to obtain 
% \daniel{
a pragmatic listener (synthesizer),
% }, 
$L_1$. Running this algorithm results in Figure. As we can see, given the utterance \textsf{\textit{01}}, this listener prefers \texttt{0+1\{1\}} over \texttt{0+1*}, reflecting the reasoning that if the user wanted to refer to \texttt{0+1*}, they might have provided an example that highlights the possibility of no 1s in the string. In this paper, we shall call this algorithm \rsaslowsingle{}. As this algorithm only depends on the meaning matrix $M$, it is applicable to all program synthesis domains where programs can be effectively enumerated and checked for consistency against examples.

\subsection{A Pragmatic Synthesizer of Multiple Examples}
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=\columnwidth]{assets/l1_2.pdf}
%     \caption{An incremental pragmatic listener that identifies \texttt{0+1\{1\}} as the most probable intended program given a second utterance \textsf{\textit{001}}. The $S_1$ distribution for this utterance builds on the distribution computed in Figure~\ref{fig:l1_1}. The utterances inconsistent with the first utterance are omitted.
%     % \daniel{a bit hard to read; embed as a PDF and maybe decrease whitespace between the three grids}
%     }
%     \label{fig:l1_2}
% \end{figure}
\begin{figure}[!h]
    \centering
    \includegraphics[width=\columnwidth]{assets/ranking-pragmatics-incremental.png}
    \caption{A boolean lexicon for a small reference game of regular expressions. The rows are the utterances (strings) and the columns are hypotheses (regexes), and each entry denotes if a string is consistent with a regex.}
    % \label{fig:incremental}
\end{figure}

\rsaslowsingle{} is capable of producing a program synthesis algorithm from a single example. However, the users will typically have to clarify their intent \emph{interactively}, by giving a sequence of multiple utterances $\mathbf{u} = u_1, u_2, \ldots, u_n$. The synthesizer must infer the intended program after every turn. This is an instance of incremental RSA \cite{incr_cohn2018incremental}, which models the informative speaker $S_1$ generating utterances auto-regressively as follows:
\begin{align*}
    S_1(\mathbf{u}|w) &= S_1(u_1, u_2, \ldots, u_n|w) \\
    &= \prod_{i=1}^{n} S_1(u_i|w, u_1, \ldots, u_{i-1}) \\
    & = \prod_{i=1}^{n} \frac{L_0(w|u_1, \ldots, u_i)}{\sum_{w'} L_0(w'|u_1, \ldots, u_i)}
\end{align*}
The synthesizer $L_1(w|u)$ is defined recursively on top of $S_1$ in the same manner as its single-utterance case.
The result of the RSA computation is shown in figure. As we can see, providing an additional utterance \textsf{\textit{001}} after the first utterance \textsf{\textit{01}} makes the incremental $L_1$ listener prefer the correct hypothesis \texttt{0+1\{1\}} even more. \cite{bool_pu2020program} builds on top of the incremental RSA algorithm with additional memoization strategies. In this work, we shall call their algorithm \rsaslow{}. Similar to \rsaslowsingle{}, this algorithm is applicable to enumerative program synthesis domains such as \citet{feser2015synthesizing,solarlezama2008sketch,gulwani2011automating}.

\subsection{Exact RSA is Slow}
\sv{shorten this to 1 paragraph ends at page 3 ideally, stick to facts and cut intuitions}
Computing $L_1$ using \rsaslow{} requires $\mathcal{O}(|W|)$ calls to $S_1$. Each call to compute $S_1$ requires $\mathcal{O}(|U|)$ calls to $L_0$, 
% \daniel{can't we compute $S_1$ once and then cache it in the computation of $L_1$? is it because it would be infeasible to do $U \times W$ consistency checks?}
which in turn requires $\mathcal{O}(|W|)$ operations to determine a set of consistent programs. 
In small domains, the results of each computation -- $L_0$, $S_1$, $L_1$ -- can be stored explicitly in matrix form, like in Figure~\ref{fig:lexicon}.
However, in incremental domains with a large number of hypotheses and utterances, it becomes infeasible to cache all the computation results explicitly, forcing the $L_1$ listener to recompute from scratch.
In practice, the pragmatic synthesizer $L_1$ runs in $\mathcal{O}(|W|^2|U|)$ time. In the incremental RSA setting with multiple (say $l$) utterances, the runtime of $L_1$ is $\mathcal{O}(|W|^2|U|l)$. As the number of hypotheses and utterances becomes large in a program synthesis domain, it becomes infeasible to compute $L_1$ at a speed required for end-user interactions. 
% For instance, \citet{vaithilingam2023usability} were only able to build a pragmatic synthesizer for the regex domain consisting of 350 regular expressions.



% explain how the synthesizer will work with a global ranking.
% show it is consistent with L1 for this example.
% do a quick runtime analysis $O(W)$ for ranking, $O(WUW)$ for L1.
% show for incremental, we can use the same order, and show it is still consistent with L1 for this example.
% show run time for this case.
% (there might be overlap with runtime analysis with this part and the next section, we'll deal with it later, just have both for now).

% the rest of the paper shows under which circumstances can this order be computed, and how to approximate if it cannot be found and blh blah.
